A Novel Falling-Ball Algorithm for Image Segmentation

Image segmentation refers to the separation of objects from the background, and has been one of the most challenging aspects of digital image processing. Practically it is impossible to design a segmentation algorithm which has 100% accuracy, and therefore numerous segmentation techniques have been proposed in the literature, each with certain limitations. In this paper, a novel Falling-Ball algorithm is presented, which is a region-based segmentation algorithm, and an alternative to watershed transform (based on waterfall model). The proposed algorithm detects the catchment basins by assuming that a ball falling from hilly terrains will stop in a catchment basin. Once catchment basins are identified, the association of each pixel with one of the catchment basin is obtained using multi-criterion fuzzy logic. Edges are constructed by dividing image into different catchment basins with the help of a membership function. Finally closed contour algorithm is applied to find closed regions and objects within closed regions are segmented using intensity information. The performance of the proposed algorithm is evaluated both objectively as well as subjectively. Simulation results show that the proposed algorithms gives superior performance over conventional Sobel edge detection methods and the watershed segmentation algorithm. For comparative analysis, various comparison methods are used for demonstrating the superiority of proposed methods over existing segmentation methods.

==> future_work.tex <==


\section{Avenues for Future Work}

As is the case with most research works, the work proposed in this paper is not without its share of limitations and scopes for improvement. The classifier used in the Falling-Ball algorithm presented in this work is a very simplified one. A better classifier is expected to yield better results of the Falling-Ball algorithm. Modifications in the fuzzy membership function used in the identification of catchment basins in the Falling-Ball algorithm may be explored to improved results. Also, the calculation of thresholding constant, which was taken as 0.11 in this work, also requires  careful attention. A bigger dataset of brain tumor images may help in the refinement of the value of this constant. Also, for images other than those of brain tumors, the calculation of the thresholding constant may be made application specific. Fuzzy method may be utilized to determine optimal threshold.
